Nuances are the Key: Unlocking ChatGPT to Find Failure-Inducing Tests with Differential Prompting

Automatically detecting software failures is an important task and a longstanding challenge. It requires finding failure-inducing test cases whose test input can trigger the software's fault, and constructing an automated oracle to detect the software's incorrect behaviors. Recent advancement of large language models (LLMs) motivates us to study how far this challenge can be addressed by ChatGPT, a state-of-the-art LLM. Unfortunately, our study shows that ChatGPT has a low probability (28.8%) of finding correct failure-inducing test cases for buggy programs. A possible reason is that finding failure-inducing test cases requires analyzing the subtle code differences between a buggy program and its correct version. When these two versions have similar syntax, ChatGPT is weak at recognizing subtle code differences. Our insight is that ChatGPT's performance can be substantially enhanced when ChatGPT is guided to focus on the subtle code difference. We have an interesting observation that ChatGPT is effective in inferring the intended behaviors of a buggy program. The intended behavior can be leveraged to synthesize programs, in order to make the subtle code difference between a buggy program and its correct version (i.e., the synthesized program) explicit. Driven by this observation, we propose a novel approach that synergistically combines ChatGPT and differential testing to find failure-inducing test cases. We evaluate our approach on Quixbugs (a benchmark of buggy programs), and compare it with state-of-the-art baselines, including direct use of ChatGPT and Pynguin. The experimental result shows that our approach has a much higher probability (77.8%) of finding correct failure-inducing test cases, 2.7X as the best baseline.

==> abstractArxiv.tex <==
\begin{abstract}
Automatically detecting software failures is an important task and a longstanding challenge. It requires finding \ftests whose test input can trigger the software's fault, and constructing an automated oracle to detect the software's incorrect behaviors. Recent advancement of large language models (LLMs) motivates us to study how far this challenge can be addressed by ChatGPT, a state-of-the-art LLM. Unfortunately, our study shows that ChatGPT has a low probability (\gptft) of finding correct \ftests for buggy programs. A possible reason is that finding \ftests requires analyzing the subtle code differences between a buggy program and its correct version. When these two versions have similar syntax, ChatGPT is weak at recognizing subtle code differences.

Our insight is that ChatGPT's performance can be substantially enhanced when ChatGPT is guided to focus on the subtle code difference. We have an interesting observation that ChatGPT is effective in inferring the intended behaviors of a buggy program. The intended behavior can be leveraged to synthesize programs, in order to make the subtle code difference between a buggy program and its correct version (i.e., the synthesized program) explicit. Driven by this observation, we propose a novel approach that synergistically combines ChatGPT and differential testing to find \ftests. We evaluate our approach on QuixBugs (a benchmark of buggy programs), and compare it with state-of-the-art baselines, including direct use of ChatGPT and Pynguin. The experimental result shows that our approach has a much higher probability (77.8\%) of finding correct \ftests, \xxxvsgptft as the best baseline.
\end{abstract}

==> rq1buggy.tex <==
\begin{table*}[]
 \caption{Effectiveness of \xxx and the baselines in finding \ftests for buggy programs of \quixbugs.}
    %\footnotesize
    \scriptsize
   \centering
    \setlength\tabcolsep{0.1pt}     % horizental space
    \def\arraystretch{0.95}
    \vspace{-2mm}
    \bgroup
 
%\renewcommand{\arraystretch}{1.2}
%    \resizebox{1.0\linewidth}{!}{
\begin{tabular}{|c||ccc|ccc|ccc|ccc|ccc|ccc|}
\toprule
                                           & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{\textbf{Failure-inducing test case that}}\\ \emph{\textbf{reports a true failure}}\\ (\emph{\ft})\end{tabular}}                                                                                                                                            & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{\textbf{Failure-inducing test case that}}\\ \emph{\textbf{reports a coincidental failure}} \\(\emph{\fc})\end{tabular}}                                                                                                             & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{\textbf{Failure-inducing test case that}}\\ \emph{\textbf{reports a false failure}} \\ (\emph{\ff})\end{tabular}}                                                                                                                    & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{\textbf{Passing test}}\\ (\emph{\pt})\end{tabular}}                                                                                                                                                                                                                                          & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\emph{\textbf{Test with Illegal}}\emph{\textbf{Arguments}} \\(\emph{\iat})\end{tabular}}                                                                                                                                                                                                                                                & \multicolumn{3}{c|}{No test case found}   \\ \hline
\emph{\textbf{Buggy programs}}             & \multicolumn{1}{c|}{\cellcolor[HTML]{83CCBC}{\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}Differential \\  Prompting\end{tabular}}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F19999}\textbf{\begin{tabular}[c]{@{}c@{}}Chat-\\ GPT\end{tabular}}} & \cellcolor[HTML]{DDB4D4}\textbf{\begin{tabular}[c]{@{}c@{}}Pyn-\\ guin\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{83CCBC}\textbf{\begin{tabular}[c]{@{}c@{}}Differential \\  Prompting\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F19999}\textbf{\begin{tabular}[c]{@{}c@{}}Chat-\\ GPT\end{tabular}}} & \cellcolor[HTML]{DDB4D4}\textbf{\begin{tabular}[c]{@{}c@{}}Pyn-\\ guin\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{83CCBC}\textbf{\begin{tabular}[c]{@{}c@{}}Differential \\  Prompting\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F19999}\textbf{\begin{tabular}[c]{@{}c@{}}Chat-\\ GPT\end{tabular}}} & \cellcolor[HTML]{DDB4D4}\textbf{\begin{tabular}[c]{@{}c@{}}Pyn-\\ guin\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{83CCBC}{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Differential \\  Prompting\end{tabular}}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F19999}{\color[HTML]{333333} \textbf{\begin{tabular}[c]{@{}c@{}}Chat-\\ GPT\end{tabular}}}} & \cellcolor[HTML]{DDB4D4}\textbf{\begin{tabular}[c]{@{}c@{}}Pyn-\\ guin\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{83CCBC}\textbf{\begin{tabular}[c]{@{}c@{}}Differential \\  Prompting\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{F19999}\textbf{\begin{tabular}[c]{@{}c@{}}Chat-\\ GPT\end{tabular}}} & \cellcolor[HTML]{DDB4D4}\textbf{\begin{tabular}[c]{@{}c@{}}Pyn-\\ guin\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Differential \\  Prompting\end{tabular} & \begin{tabular}[c]{@{}l@{}}Chat-\\ GPT\end{tabular} & \begin{tabular}[c]{@{}l@{}}Pyn-\\ guin\end{tabular} \\ \hline \hline
bitcount                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}                                & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                               & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0 \\ \hline
breadth-first-search                       & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}  \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}  \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                                              & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
bucketsort                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0}  \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0}  \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}                                                                           & \multicolumn{1}{c|}{3}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
depth-first-search                         & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 9}}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                                             & \multicolumn{1}{c|}{7}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
detect-cycle                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                               & \multicolumn{1}{c|}{9}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
find-first-in-sorted                       & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                                                      & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
find-in-sorted                             & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{EEEED1} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                                                                  & \multicolumn{1}{c|}{4}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
flatten                                    & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                               & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
gcd                                        & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                                & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
get-factors                                & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}}                                        & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 9}}                                                                                        & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
hanoi                                      & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                                          & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
v-parenthesization                         & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                                                        & \multicolumn{1}{c|}{3}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
kheapsort                                  & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                                          & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
knapsack                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                                       & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
kth                                        & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8} }                                                                                  & \multicolumn{1}{c|}{3}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
lcs-length                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} {\color[HTML]{000000} 2}}}                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{EEEED1}\color[HTML]{000000} 3}                                                                                         & \multicolumn{1}{c|}{2}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
levenshtein                                & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                                         & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
lis                                        & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0}\color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                                 & \multicolumn{1}{c|}{2}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
c-subsequence                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 9}}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                             & \multicolumn{1}{c|}{2}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
max-sublist-sum                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                               & \multicolumn{1}{c|}{3}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
mergesort                                  & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                                             & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
spanning\_tree                             & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                               & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
next\_palindrome                           & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                               & \multicolumn{1}{c|}{10}                                                                                                                & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
next\_permutation                          & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 9}}}                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                                                                               & \multicolumn{1}{c|}{1}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
pascal                                     & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                                               & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
possible\_change                           & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                             & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
powerset                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                                             & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
quick\_sort                                & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                                               & \multicolumn{1}{c|}{7}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
reverselinkedlist                          & \multicolumn{1}{c|}{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}                                & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                                             & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
rpneval                                    & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 9}}}                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}                                                                          & \multicolumn{1}{c|}{1}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
s\_path\_length                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1}\color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}                                                                              & \multicolumn{1}{c|}{8}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
s\_path\_lengths                           & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} \color[HTML]{FFFAFA} 10}}}         & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA}\color[HTML]{FFFAFA} 8}}                                                         & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
shortest\_paths                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                               & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
shunting\_yard                             & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}} }                             & \multicolumn{1}{c|}{\cellcolor[HTML]{CDCDB4} {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                      & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
sieve                                      & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                                                                               & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
sqrt                                       & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}}}                              & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                                        & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 9}}                                                                             & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
subsequences                               & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}}                                        & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                                                                               & \multicolumn{1}{c|}{10}                                                                                                                & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
to\_base                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 10}} }                             & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{8B8B7A} {\color[HTML]{FFFAFA} 8}}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 4}                                                                             & \multicolumn{1}{c|}{0}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
topological\_ordering                      & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                               & \multicolumn{1}{c|}{10}                                                                                                                & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
wrap                                       & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}}                                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                 & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                                                   & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                        & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                 & \multicolumn{1}{c|}{{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}}                                                                            & \multicolumn{1}{c|}{{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}}                 & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                                               & \multicolumn{1}{c|}{4}                                                                                                                 & \multicolumn{1}{c|}{0}                                                      & 0\\ \hline
\emph{\textbf{Average}}                    & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{7.5}}                                             & \multicolumn{1}{c|}{ \cellcolor[HTML]{FFC1C1} \textbf{2.9}}                                      & \cellcolor[HTML]{FFC1C1} \textbf{0.8}                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.2}}                                                                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{1.9}}                                      & \cellcolor[HTML]{FFC1C1} \textbf{0.2}                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.0}}                                                                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.8}}                                      & \cellcolor[HTML]{FFC1C1} \textbf{0.0}                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.0}}                                                                                                                        & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{3.0}}                                                             & \cellcolor[HTML]{FFC1C1} \textbf{3.2}                                      & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.0}}                                                                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{1.5}}                                      & \cellcolor[HTML]{FFC1C1} \textbf{5.6}                                      & \multicolumn{1}{c|}{2.2}                                                              & \multicolumn{1}{c|}{0}       & 0 \\ \bottomrule
\multicolumn{16}{l}{$^\dag$\emph{Each cell of the table shows the number of \ft, \fc, \ff, \pt and \iat found by \xxx and the baselines for each buggy programs of {\mycode QuixBugs}.}}\\
\multicolumn{16}{l}{$^\dag$\emph{For each program, \xxx and the baselines are run ten times.}}\\
\end{tabular}
%}
%
\vspace{-6mm}
\egroup
\label{tab:rq1buggy}
\end{table*}

==> rq1correct.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[]
\begin{table*}[]
 \caption{Effectiveness of \xxx and the baselines in finding \ftests for correct programs of \quixbugs.}
 	\scriptsize
   %\footnotesize
   \centering
    \setlength\tabcolsep{7pt}     % horizental space
    \def\arraystretch{ 1}
    \vspace{-2mm}
    \bgroup
 
%\renewcommand{\arraystretch}{1.2}
 %   \resizebox{1.0\linewidth}{!}{
\begin{tabular}{|c||ccc|ccc|ccc|}
\toprule
                           & \multicolumn{ 3}{c|}{\begin{tabular}[c]{@{}c@{}} \emph{\textbf{Failure-inducing test case that}}\\ \emph{\textbf{reports a false failure}} (\emph{\ff})\end{tabular}}                                                                                                                                      & \multicolumn{ 3}{c|}{\emph{\textbf{Passing test}} (\emph{\pt})}                                                                                                                                                                                          & \multicolumn{ 3}{c|}{\emph{\textbf{Test with Illegal Arguments}} (\emph{\iat})}                                                                                                                                                             \\ \hline
                        \multicolumn{ 1}{|c||}{ \emph{\textbf{Buggy programs}} }  & \multicolumn{ 1}{c|}{\cellcolor[HTML]{83CCBC}{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\emph{Differential} \\  \emph{Prompting}\end{tabular}}} & \multicolumn{ 1}{c|}{\cellcolor[HTML]{F19999}{\color[HTML]{333333} \emph{ChatGPT}}} & \cellcolor[HTML]{DDB4D4}\emph{\textsc{Pynguin}} & \multicolumn{ 1}{c|}{\cellcolor[HTML]{83CCBC}{\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}\emph{Differential} \\  \emph{Prompting}\end{tabular}}} & \multicolumn{ 1}{c|}{\cellcolor[HTML]{F19999}\emph{ChatGPT}} & \cellcolor[HTML]{DDB4D4}\emph{\textsc{Pynguin}} & \multicolumn{ 1}{c|}{\cellcolor[HTML]{83CCBC}\begin{tabular}[c]{@{}c@{}}\emph{Differential} \\  \emph{Prompting}\end{tabular}} & \multicolumn{ 1}{c|}{\cellcolor[HTML]{F19999}\emph{ChatGPT}} & \cellcolor[HTML]{DDB4D4}\emph{\textsc{Pynguin}} \\ \hline \hline
bitcount                   & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               \\ \hline
breadth-first-search       & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               \\ \hline
bucketsort                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              \\ \hline
depth-first-search         & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
detect-cycle               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               \\ \hline
find-first-in-sorted       & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               \\ \hline
find-in-sorted             & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               \\ \hline
flatten                    & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
gcd                        & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
get-factors                & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
hanoi                      & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
valid-parenthesization  & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               \\ \hline
kheapsort                  & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               \\ \hline
knapsack                   & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               \\ \hline
kth                        & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              \\ \hline
lcs-length                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
levenshtein                & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               \\ \hline
lis                        & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
common-subsequence & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
mergesort                  & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               \\ \hline
spanning\_tree    & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               \\ \hline
next\_palindrome           & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                                                     & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               \\ \hline
next\_permutation          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               \\ \hline
pascal                     & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               \\ \hline
possible\_change           & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              \\ \hline
powerset                   & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               \\ \hline
quick\_sort                & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               \\ \hline
reverselinkedlist          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
rpneval                    & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              \\ \hline
shortest\_path\_length     & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                         & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
shortest\_path\_lengths    & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
shortest\_paths            & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
shunting\_yard             & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                               \\ \hline
sieve                      & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 10}                              & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
sqrt                       & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
subsequences               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
to\_base                   & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                               & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 2}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 8}                               \\ \hline
topological\_ordering      & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 5}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 3}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               \\ \hline
wrap                       & \multicolumn{ 1}{c|}{\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 7}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{8B8B7A} \color[HTML]{FFFAFA} 9}                                                      & {\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                                                 & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                               & {\cellcolor[HTML]{CDCDB4} \color[HTML]{000000} 6}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 0}                                                                                          & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFFFE0} \color[HTML]{000000} 1}                               & {\cellcolor[HTML]{EEEED1} \color[HTML]{000000} 4}                               \\ \hline
\textit{\textbf{Average}}                    & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.3} }                                                                                                              & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{2.2} }                                                   & \cellcolor[HTML]{FFC1C1} \textbf{0.0}                               & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.0}}                                                                                                                & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{7.2}}                             & \cellcolor[HTML]{FFC1C1} \textbf{3.3}                             & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.0}}                                                                                        & \multicolumn{ 1}{c|}{\cellcolor[HTML]{FFC1C1} \textbf{0.4}}                             & \cellcolor[HTML]{FFC1C1} \textbf{6.7}                             \\ \bottomrule
\multicolumn{ 10}{l}{$^\dag$\emph{Each cell of the table shows the number of \ft, \fc, \ff, \pt and \iat found by \xxx and the baselines for each buggy programs of {\mycode QuixBugs}.}}\\
\multicolumn{ 10}{l}{$^\dag$\emph{For each program, \xxx and the baselines are run ten times.}}\\
\end{tabular}
\egroup
\vspace{-4mm}
\label{tab:rq1correct}
\end{table*}

